Generative Minimization Networks: Training GANs Without Competition

Many applications in machine learning can be framed as minimization problems and solved efficiently using gradient-based techniques. However, recent applications of generative models, particularly GANs, have triggered interest in solving min-max games for which standard optimization techniques are often not suitable. Among known problems experienced by practitioners is the lack of convergence guarantees or convergence to a non-optimum cycle. At the heart of these problems is the min-max structure of the GAN objective which creates non-trivial dependencies between the players. We propose to address this problem by optimizing a different objective that circumvents the min-max structure using the notion of duality gap from game theory. We provide novel convergence guarantees on this objective and demonstrate why the obtained limit point solves the problem better than known techniques.

==> broader_impact.tex <==
\section*{Broader Impact}

GANs have raised a lot of interest in the machine learning community due to their potential to be used as a tool in various scientific fields, including e.g. in photo editing, cosmology, etc. Unfortunately, training a GAN can still prove to be challenging and most often requires expert knowledge to properly tune the training algorithm's hyperparameters. Most training methods exhibit potentially pathological behaviors (such as the cyclic behavior described in our paper) which can lead to divergence or convergence to a suboptimal set of parameters. Our research focuses on addressing such problems by defining a new objective function which we show empirically to address many of the training problems exhibited by alternative training methods.

From a societal point of view, we believe that a positive impact of our research is that it will yield to new developments of GANs in novel domains. However, we do acknowledge that deep generative models can be used to produce synthetic images and videos for false news stories.

I - Capabilities

\paragraph{Applications of GANs.}
Currently, the main applications of GANs fall within the image domain (generation of high-quality images, image inpainting, super-resolution, person re-identification, object detection, video prediction and generation, facial attribute manipulation, anime character generation, image to image translation, text to image translation, face aging, human pose estimation, de-occlusion and image blending). However, the interest of using GANs for other domains is actively rising. In particular, we are starting to see research using GANs for text, cosmology, domain adaptation, speech and music, drug discovery, reinforcement learning, games, machine learning security, adversarial mechanisms for preserving privacy, and adversarial mechanisms for cryptography among others.

\paragraph{Effects of this research on applications.}
This paper provides a novel method for training GANs that circumvents the adversarial nature of the game and instead offers a common objective for both players to minimize. By doing so, we show that the models exhibit more stable behaviour and convergence properties. In addition, we have shown that one can take pretrained GAN models and continue training them with our objective, resulting in increased performance in the resulting models. Finally, our algorithm is less sensitive to the choice of hyperparameters than alternative methods, which may lead to decreased time of hyperparameter tuning.

\paragraph{Impact on research.}
Our work could increase the rate of progress within a domain such as images, but is not limited to the image domain only. Concretely, the algorithm we propose can be used as a replacement of standard methods as a more stable alternative or to further improve already pretrained models, thus advancing the ability of GANs to generate high fidelity samples. 

II - Implications

\paragraph{Societal impacts of uses.}
There are many positive potential use-cases of GANs -- such as drug discovery and molecular development, the production of art and entertainment, and, more speculatively, cryptography. Furthermore, there are many areas (in particular medicine) where data is scarce and data augmentation is thus crucial for training ML models. GANs can be particularly useful for that task and enable the otherwise impossible employment of ML models in different areas. However, there are several widely discussed negative uses of GANs, such as in their use to produce synthetic images and videos for false news stories, scams, and pornographic media involving the faces of people who did not consent. Furthermore, audio synthesis could lead to new methods of impersonating specific people. Overall, the biggest potential negative effect that we can foresee for GANs is that GANs can be used as a tool for those wishing to spread misinformation or create an environment of uncertainty and mistrust. Deepfakes may lead to a general mistrust of the population given that it could be hard to distinguish what is real and what is not. The long term impacts of synthetic media is highly uncertain. However, such uses may become more widespread as GANs become increasingly data efficient.


III - Initiatives

\paragraph{Future work to help.} 
Potential ways to stay on top of the usage of GANs for deepfakes, and overall for negative applications, could be to start new research (directions) into detection systems for problematic synthetic content. To further incentivise such work, there could be benchmarks, competition and fundings to be organised.
